Complexity of Paired Domination Problems on Circle and $k$-Polygon Graphs

A set $D \subseteq V$ is a dominating set of a graph $G$ if every vertex in $V - D$ is adjacent to at least one vertex in $D$. A dominating set $D$ is a paired-dominating set if the subgraph of $G$ induced by $D$ contains a perfect matching. In this paper, we prove that determining the minimum paired-dominating set in circle graphs is NP-complete. We further present an $O(n(\frac{n}{k^2-k})^{2k^2-2k})$-time algorithm for finding the minimum paired-dominating set in $k$-polygon graphs, a subclass of circle graphs. Additionally, we refine the existing algorithm of Elmallah and Stewart for computing the minimum dominating set in $k$-polygon graphs, reducing its time complexity from $O(n^{4k^2+3})$ to $O(n^{3k-5})$, and further extend it to find the minimum total dominating set.

==> total_transformation.tex <==
            \tikzset{
                vertex/.style ={circle, draw=black, fill=white, thick, minimum size=7mm, inner sep=2pt}
            }
            \draw node[vertex] (a) at(0, 4*0.8) {$a$};
            \draw node[vertex] (b) at(0, 2*0.8) {$b$};
            \draw node[vertex] (c) at(-1, 2 - 1.732) {$c$};
            \draw node[vertex] (d) at(1, 2 - 1.732) {$d$};
            \draw [thick] (a)--(b);
            \draw [thick] (b)--(c);
            \draw [thick] (c)--(d);
            \draw [thick] (d)--(b);
            \draw node (tmp) at(0, -0.2) {};




            \tikzset{
                vertex/.style ={circle, draw=black, fill=white, thick, minimum size=7mm, inner sep=2pt}
            }
            \def\bias {4}
            \draw [thick] (-1+\bias, 2 - 1.732) parabola bend (2+\bias,-0.4) (5+\bias, 2 - 1.732);
            \draw [thick] (1+\bias, 2 - 1.732) parabola bend (2+\bias,-0.1) (3+\bias, 2 - 1.732);
            \draw node[vertex] (al) at(0+\bias, 4*0.8) {$a_\ell$};
            \draw node[vertex] (bl) at(0+\bias, 2*0.8) {$b_\ell$};
            \draw node[vertex] (cl) at(-1+\bias, 2 - 1.732) {$c_\ell$};
            \draw node[vertex] (dl) at(1+\bias, 2 - 1.732) {$d_\ell$};
            \draw node[vertex] (ar) at(4+\bias, 4*0.8) {$a_r$};
            \draw node[vertex] (br) at(4+\bias, 2*0.8) {$b_r$};
            \draw node[vertex] (cr) at(3+\bias, 2 - 1.732) {$c_r$};
            \draw node[vertex] (dr) at(5+\bias, 2 - 1.732) {$d_r$};
            \draw [thick] (al)--(bl); \draw [thick] (ar)--(br);
            \draw [thick] (bl)--(cl); \draw [thick] (br)--(cr);
            \draw [thick] (cl)--(dl); \draw [thick] (cr)--(dr);
            \draw [thick] (dl)--(bl); \draw [thick] (dr)--(br);
            \draw [thick] (al)--(br); \draw [thick] (ar)--(bl);
            \draw [thick] (bl)--(cr); \draw [thick] (br)--(cl);
            \draw [thick] (dl)--(br); \draw [thick] (dr)--(bl);
            \draw node (tmp) at(0, -0.2) {};


            \node (label_a) at (0,-1.08) {$(a)$};
            \node (label_b) at (2+\bias,-1.08) {$(b)$};

